Fine structure splitting analysis of cavity-enhanced telecom-wavelength InAs quantum dots grown on a GaAs(111)A vicinal substrate

The effcient generation of entangled photons at telecom wavelength is crucial for the success of many quantum communication protocols and the development of fiber-based quantum networks. Entangled light can be generated by solid state quantum emitters with naturally low fine structure splitting, such as highly symmetric InAs quantum dots (QDs) grown on (111)-oriented surfaces. Incorporating this kind of QDs into optical cavities is critical to achieve sufficient signal intensitiesfor applications, but has so far shown major complications. In this work we present droplet epitaxy of telecom-wavelength InAs QDs within an optical cavity on a vicinal (2{\deg} miscut) GaAs(111)A substrate. We show a remarkable enhancement of the photon extraction efficiency compared to previous reports together with a reduction of the density that facilitates the isolation of single spectral lines. Moreover, we characterise the exciton fine structure splitting and employ numerical simulations under the framework of the empirical pseudopotential and configuration interaction methods to study the impact of the miscut on the optical properties of the QDs. We demonstrate that the presence of miscut steps influences the polarisation of the excitonic states and introduces a preferential orientation in the $C_{3v}$ symmetry of the surface.

==> Section_4/Section_4.tex <==
\section{Fine structure splitting orientation}
%
\begin{figure*}
\includegraphics[width=0.7\textwidth]{Figures/polar_plots_fig_alloy_v3.pdf}
\caption{Polar diagrams showing the square of the optical transition dipole matrix element calculated for GaAs/AlAs (top panel), GaAs/Al\textsubscript{0.15}Ga\textsubscript{0.85}As (middle panel) and InAs/GaAs (bottom panel) QDs assuming different values of the miscut angle $\alpha$. X\textsubscript{LOW} (X\textsubscript{HIGH}) represents the lowest (highest) lying bright exciton state in energy. When two exciton bright states are degenerate, they are labelled X\textsubscript{B}.
\label{Fig3} }
\end{figure*}
%
%
\noindent The measurements summarized in Figure \ref{Fig2}b revealed the presence of emitters with large (> 100 $\mu$eV) FSS, which can be related the presence of unexpected stress and anisotropy in some of the QDs examined. In order to shed light on this phenomenon, we carried out an additional investigation after adjusting the position of the sample in the cryostat such that it was possible to identify the direction of the miscut steps with respect to the lab frame and to the optics mounted in the collection arm of the confocal microscope. In this arrangement, light emitted from a QD and polarized along the (112) direction would be transmitted through the LP for a HWP rotation of 82\textdegree.
We repeated the FSS characterization over 35 new emitters, confirming the previous result of FSS < 100 $\mu$eV in approximately 50\% of the cases. Moreover, for the majority of the QDs the oscillations of the energy offset are found to follow a specific pattern, showing the first maximum for a similar HWP rotation as summarized in \ref{Fig2}c.  of approximately 82\textdegree.
the QDs tend to have dipoles aligned along the direction of the miscut steps.
\\Interestingly, a small group of QDs 
These results suggest that the polarization of the excitonic transitions follows a preferential orientation dependent on the direction of the miscut steps.
%


